PowerSimulationsDynamics.jl -- An Open Source Modeling Package for Modern Power Systems with Inverter-Based Resources

In this paper we present the development of an open-source simulation toolbox, PowerSimulationsDynamics.jl, to study the dynamic response of power systems, focusing on the requirements to model systems with high penetrations of Inverter-Based Resources (IBRs). PowerSimulationsDynamics.jl is implemented in Julia and features a rich library of synchronous generator, inverter, and load models. In addition, it allows the study of quasi-static phasors and electromagnetic dq models that use a dynamic network representation. Case studies and validation exercises show that PowerSimulationsDynamics.jl results closely match other commercial and open-source simulation tools.

==> figs/eigs_plot.tex <==
\begin{figure}[H]
    %\centering
    \begin{tikzpicture}
    \begin{semilogxaxis}[xlabel=$\text{Re}(\lambda)$,
    ylabel=$\text{Im}(\lambda)$,
    xmin=10,
    xmax=10000,
    ymin=-10000,
    ymax=10000,
    width=3.0in,
    height=2.5in,
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},
    xmajorgrids=true,
    ymajorgrids=true,
    ytick = {-10000, -5000, 0, 5000, 10000},
    yticklabels={$-10^4$,$-5 \cdot 10^{3}$,$0$,$5 \cdot 10^3$,$10^4$},
    grid style=dashed,
    scaled y ticks = false, 
    legend style={at={(0.45,0.15)},anchor=south east,draw=none, font=\footnotesize}]
    \addplot [color=blue, only marks, mark=o, mark size = 2.2pt] table [col sep=comma] {data/eigs_pscad_neg.csv};
    \addplot [color=red, only marks, mark=x, mark size = 2.5pt] table [col sep=comma] {data/eigs_dyn_pscad_neg.csv};
    \legend{Algebraic Lines, Dynamic Lines}
    \end{semilogxaxis}
    \end{tikzpicture}
\end{figure}

